Multilevel Weighted Support Vector Machine for Classification on Healthcare Data with Missing Values

This work is motivated by the needs of predictive analytics on healthcare data as represented by Electronic Medical Records. Such data is invariably problematic: noisy, with missing entries, with imbalance in classes of interests, leading to serious bias in predictive modeling. Since standard data mining methods often produce poor performance measures, we argue for development of specialized techniques of data-preprocessing and classification. In this paper, we propose a new method to simultaneously classify large datasets and reduce the effects of missing values. It is based on a multilevel framework of the cost-sensitive SVM and the expected maximization imputation method for missing values, which relies on iterated regression analyses. We compare classification results of multilevel SVM-based algorithms on public benchmark datasets with imbalanced classes and missing values as well as real data in health applications, and show that our multilevel SVM-based method produces fast, and more accurate and robust classification results.

==> Medicalintro.tex <==
\section{The role of predictive modeling in healthcare}
Modern healthcare can be characterized as \textit{evidence-driven} and \textit{model-assisted} \cite{foldy2014national}. In an ideal situation, every decision in the clinical environment should be supported by a statistical predictive model for risks and possible outcomes. This model may have a form of a simplified risk-assessment formula \cite{haas2013risk}, or a sophisticated machine learning tool \cite{plis2014machine}, \cite{woolery1994machine}. In either case, the model is based on a query from a database containing relevant examples from medical and operational history. 

In practice, comprehensive medical information is stored in  separate databases, with different formats and rules of access. Due to considerations of patient privacy, and the proprietary nature of electronic medical records \cite{larson2004survey}, the databases cannot be queried continuously. Every instance of data acquisition and integration is a separate effort that is cost-effective only when the resulting predictive model shows very high quality. Thus, progress in evidence-driven healthcare depends on how well state-of-the art algorithms of machine learning are adapted to clinical data.

We note that classical computer science issues, such as scalability, or convergence rate are rarely an issue in machine learning for healthcare. Instead, an algorithm is ranked based on its ability to process raw medical data, with such problematic features as sparsity (including accidentally missing data) and imbalanced outputs. Massive medical data is inherently sparse because of the encounter nature of patient-hospital interaction. When a clinical encounter occurs, some labels are attached to it \cite{snomed2011systematized}; the number and contents of labels vary widely, and at all other times the state of the patient is unknown. The outcomes of interest in classification problems are inherently imbalanced because, as a rule, healthcare analytics is motivated by data with evidence of crisis, severe health conditions, gaps and bottlenecks in access to care, all of these are rare events.

Many of such issues are not obvious from the perspective of a local healthcare provider (such as a single doctor); by definition they have access to all knowledge they ever use. We view this paper as a short, high-level primer on using advanced methods of machine learning to overcome the difficulties that emerge after multiple datasets are integrated for analysis and prediction.

This work was prompted by several projects completed with the Division of Applied Research and Clinical Informatics, Dept. of Data Science; Geisinger Health System. The routine activity of Data Science consists of medium-scope predictive projects on a combination of patient biometrics, pathology lab results, clinical encounter data, medical insurance data (available directly from Geisinger Health Plan) and externally assigned aggregate metrics for patients' general lifestyle risks, compliance with treatment regime, and loyalty to a particular provider. 

For the first motivating example, we use our 2014 feasibility study \cite{RoderickMEDAI} of merging insurance information (6 aggregate features, based on the history of claims and payments) together with clinical encounter information (10-20 features chosen by hand from patient biometrics, medications and diagnostic codes). The goal of the initial study was to predict the financial risk for a particular patient (a common metric in insurance practice, derived as a ratio of individual expenses and average expenses for a large demographic group). Furthermore, we wanted to see how addition of the clinical information changes the predictive power of the model, thus making a case for existence of high-risk patients that are invisible to claims-based analysis. We used a standard clustering technique, k-nearest neighbors with empirically selected weighting, to achieve the basic results.

For the second example, we use our preliminary investigation of patients' response to public outreach \cite{RoderickFLU}, such as annual flu awareness campaigns. We included basic demographic and clinical information on patients targeted by 35 such campaigns into the model predicting whether a given patient is likely to respond to the reminder, or to choose not to get vaccinated, or use a different provider. Again, our core predictive model was standard: logistic regression with empirically selected weighting of training data.

We now pose a question: how much more effective would the predictive models be in each case with the use of an advanced machine learning algorithm developed with awareness of sparsity and class skewness (imbalance) in data?

\section*{Additional notes}

Note: use this for the numerical results section.

The first table is based on Example 1, a classification task of placing a patient in a correct group by financial risk (ordered from 1 to 5). The motivation of the original study was to determine how much integration of the medical and financial data changes the outcomes of clustering and classification operations based on financial data alone. For that purpose, modest precision was sufficient; we used a logistic (linear) regression approach (implemented as \textit{mnrfit} in Matlab). We are comparing the precision of with the best results obtained by multilevel support vector machine method.

\begin{tabular}{|c|c|c|c|c|c|}
	\hline Class of financial risk & 1 & 2 & 3 & 4 & 5 \\ 
	\hline Precision using logistic regression & 0.58 & 0.54 & 0.53 & 0.51 & 0.59 \\ 
	\hline Precision using SVM & 0.73 & 0.50 & 0.44 & 0.50 & 0.71 \\ 
	\hline 
\end{tabular} 

To interpret the results, please note that correct identification of intermediate risk categories is a very difficult problem in medical informatics. To our knowledge, there is no good definition of "average health", either evidence-driven or philosophical, that would help an expert to identify such patient features that do not indicate an acute crisis, or an almost certain safety from crisis. Accordingly, it is not surprising that neither approach does well on the risk categories 2..4; there is also not a lot of motivation to improve the model there.
On the other hand, it is important to identify and predict the very low-risk patients (knowing that status ahead of time allows resource re-allocation leading to savings and improved service for everyone) and the very high-risk patients (so that clinical and financial resources could be prepared for the forthcoming crisis).

Accordingly, it is important that the use of an advanced method of machine learning changes the quality of prediction from almost worthless ('toss a coin') to workable (precision of $0.7$). 

In the second table, we are comparing results for the basic approach and a support vector machine prediction for Example 2, a study of patient's response to hospital flu outreach. This example involves a binary classifier: either the patient will get vaccinated after reminder, or not (this includes using a different provider) In the preliminary study, we used adaptive linear regression model (LASSO for adaptive selection of features, logistic regression on actual prediction). We compare with two versions of SVM.

\begin{tabular}{|l|l|l|l|}
	\hline  & Sensitivity  & Specificity & Accuracy \\ 
	\hline Adaptive logistic regression & 0.8903 & 0.6345 & 0.7619 \\ 
	\hline Standard SVM & 0.9750 & 0.6583 & 0.8496 \\ 
	\hline Weighted SVM & 0.9739 & 0.6598 & 0.8495 \\ 
	\hline 
\end{tabular} 

Response to outreach is not a crucial life-or-death issue, we are performing this study to see if predictive modeling can assist with resource allocation (which patients to contact, how much medical personnel effort to dedicate to outreach and then vaccination). Arguably, accuracy is more important than specificity here. 
Even the basic results (using linear regression) were met with approval the CPSL (Care Patient Service Line: a division responsible for coordinating efforts of local, small-scale healthcare providers operating under Geisinger). SVM methods (almost 10 percent improvement) provide additional justification for the use of machine learning on merged data to assist planning in clinical practice.

